A Theory of Composable Lingos for Protocol Dialects

Formal patterns are formally specified solutions to frequently occurring distributed system problems that are generic, executable, and come with strong qualitative and/or quantitative formal guarantees. A formal pattern is a generic system transformation which transforms a usually infinite class of systems in need of the pattern's solution into enhanced versions of such systems that solve the problem in question. In this paper we demonstrate the application of formal patterns to protocol dialects. Dialects are methods for hardening protocols so as to endow them with light-weight security, especially against easy attacks that can lead to more serious ones. A lingo is a dialect's key security component, because attackers are unable to ''speak'' the lingo. A lingo's ''talk'' changes all the time, becoming a moving target for attackers. In this paper we present several formal patterns for both lingos and dialects. Lingo formal patterns can make lingos stronger by both transforming them and by composing several lingos into a stronger lingo. Dialects themselves can be obtained by the application of a single dialect formal pattern, generic on both the chosen lingo and the chosen protocol.

==> text/preliminaries.tex <==
We summarized background on Maude and Actor systems relevant for this paper.

% Maude
\noindent {\bf Maude} \cite{maude-book,duran_programming_2020} is a formal specification language and system based on rewriting 
logic~\cite{MeseguerTCS92,20-years}, a logic for specifying a wide range of concurrent systems, including, e.g.,
Petri nets \cite{stehr-meseguer-olveczky}, process calculi \cite{Verdejo-Marti-Oliet00}, object-based systems \cite{ooconc}, asynchronous hardware \cite{DBLP:journals/jlp/KatelmanKM12}, mobile ad hoc network protocols \cite{liu-etal-MANETS-JLAMP}, cloud-based storage systems \cite{cloud-chapter}, web browsers \cite{IE-maude-analysis}, concurrent programming languages \cite{meseguer-rosu-tcs}, distributed  control systems \cite{multirate-pals-SCP} and models of mammalian cell pathways \cite{pathways02,pathways04}.  A rewite theory is a triple $\mathcal{R}=(\Sigma,E,R)$,
where $(\Sigma,E)$ is an equational theory defining the system states as elements of the initial algebra
$T_{\Sigma/E}$, and $R$ is a collection of rewrite rules
of the form $t \rightarrow t'$ that describe the local concurrent transitions of the
concurrent system specified by $\mathcal{R}$.

% Functional modules
\noindent {\bf Maude Functional (resp. System) Modules and Theories}. Rewriting Logic has Equational Logic as a sublogic. 
In Maude this corresponds to the sublanguage of \emph{functional modules and theories}.  
A  Maude \emph{functional module} is an equational theory $(\Sigma,E)$ delimited with keywords \texttt{fmod} and \texttt{endfm}
and having an \emph{initial algebra semantics}, namely, $T_{\Sigma/E}$.  It includes type and operator declarations
for $\Sigma$ (with the \texttt{sort}, resp. \texttt{op}, keywords), and equations $E$ declared with the \texttt{eq} keyword. Users can declare their own operator's syntax with '\texttt{\_}' denoting argument positions, e.g., \texttt{\_+\_} specifies a binary infix symbol. Maude binary operators can be specified with built-in equational attributes such as associativity (\texttt{assoc}), commutativity (\texttt{comm}) and identity (\texttt{id:}).
Likewise, a Maude \emph{functional theory} is an equational theory $(\Sigma,E)$ delimited by keywords \texttt{fth} and \texttt{endfth} 
with a \emph{loose semantics} (specifies all algebras satisfying the theory).
Similarly, a Maude \emph{system module} (resp. \emph{system theory}) is a rewrite theory $(\Sigma,E,R)$
delimited with keywords \texttt{mod} and \texttt{endm} (resp. \texttt{th} and \texttt{endth})
with an \emph{initial} (resp. \emph{loose}) model semantics.  The rules $R$ in a system module (resp, theory)
are introduced with the keyword \texttt{rl}.
See \cite{maude-book,maude-manual} for further details.

% Parameterised programming
\noindent {\bf Maude Parameterized Modules}.
Maude supports \emph{parameterized functional modules}  having a \emph{free algebra semantics}.
They are parameterized by one of more functional theories.  For example, \verb+fmod MSET{X :: TRIV} endfm+
is a parameterized module with parameter theory \texttt{TRIV} having a single parameter type \texttt{Elt} and no
operations or equations that maps any chosen set $X$ of elements to the free algebra of (finite) multisets on the elements
of $X$.  The choice of an actual parameter $X$ is made by a Maude \emph{view} instantiating in this case 
\texttt{TRIV} to the chosen data type $X$.  For example, we can choose as elements the natural numbers
by a view \texttt{Nat} mapping \texttt{TRIV} to the functional module \texttt{NAT} of natural numbers
and mapping the parameter type (called a sort) \texttt{Elt} to the type (sort) \texttt{Nat} in \texttt{NAT}.
The semantics of the thus instantiated module \verb+fmod MSET{Nat}+ is the free algebra
of multisets with elements in the natural numbers.  
%
% A more interesting example
% is a parameterized module \verb+fmod POLY{R :: RING, X :: TRIV} endfm+
% of polynomials, which can be instantiated to obtain polynomials on any chosen ring of coefficients and any chosen set of variables
% by suitable views from \texttt{RING} and \texttt{TRIV}.
% For example, \verb+fmod POLY{Int,Qid}+ can define the algebra of polynomials with integer coefficients and
% quoted identifiers as variables.  
%
Likewise, \emph{parameterized system modules}  have a \emph{free model semantics}.
For example, a parameterized system module \verb+mod CHOICE{X :: TRIV} endm+ that imports 
the parameterized functional module \verb+fmod MSET{X :: TRIV} endfm+ can have a  rewrite rule
for non-deterministically choosing an element
in a multiset of elements.  Then, the instantiation \verb+mod CHOICE{Nat} endm+ provides non-deterministic
choice of an element in a multiset of natural numbers.


% Generalised Actor Systems
\noindent {\bf Actors} \cite{Agha86} model distributed systems in which  distributed objects communicate through asynchronous message passing. When an actor receives a message, it changes its state, may send new messages, and may create new actors. 
In \cite{DBLP:journals/pacmpl/LiuMOZB22,ProtocolDialects-FormalPatterns}, actors have been extended to 
\emph{generalized actor rewrite theories} (GARwThs). These are object-oriented rewrite theories 
specified in Maude as a special class of system modules
that satisfy natural requirements. 
The distributed states of a GARwTh (terms of sort \texttt{Configuration}) are multi-sets of objects (terms of sort \texttt{Object}) and messages (terms of sort \texttt{Msg}). Multiset union is modelled by an associative and commutative operator `\verb!_ _!' ( juxtaposition), with \texttt{null} is the empty multi-set. Communication protocols are typical GARwThs.

% MQTT formal semantics
\subsection{Formal Semantics of MQTT} \label{subsec:MQTT}

MQTT ~\cite{HunkelerTS08} is a lightweight, publish-subscribe, protocol %that incorporates some message queuing services and is 
popular in devices with limited resources or network bandwidth. %, such as the Internet of Things (IoT), indeed it is recommended as part of the ISO/IEC 20922.
It requires a transport protocol such as TCP/IP that can provide ordered, lossless, bi-directional connections.  MQTT provides no security itself, and, although it can be run over secure transport protocols such as TLS, it is known to be commonly misconfigured \cite{hron20189mqtt}. This makes it an attractive application for protocol dialects%, see for example 
\cite{gogineniverify}. We use MQTT as the base protocol for the examples shown in the paper. 

\begin{example}\label{ex:MQTT-formal-semantics}
We formalize MQTT in Maude as a protocol example for Dialects. Specifically, we select to specify a subset of MQTT for illustration purposes. We give formal semantics to the following MQTT commands: connect, subscribe, unsubscribe, publish and disconnect. Furthermore, in our MQTT's symbolic model we have two classes of actors, \texttt{MqttClient} and \texttt{MqttBroker}. Class \texttt{MqttClient} defines three attributes: i) the broker it is connected to, ii) a list of commands to execute in order, and iii) a map between topic and value, to store the last value received on the subscribed topic. Class \texttt{MqttBrocker} has two attributes: i) a lists of peers and ii) a map between topics and the peers subscribed to it. With these two classes and set of commands we can build and represent environments with multiple clients and brokers, exchanging messages in a concurrent and asynchronous manner. 

As an example of the formal semantics of MQTT, we show the process of a client connecting to a broker with the actor rules of Figure~\ref{fig:mqtt-actor-rules}. First rule models the behaviour of an \texttt{MqttClient} with identifier \texttt{Me} sending a \texttt{connect} message to an \texttt{MqttBroker} with identifier \texttt{B}. Second rule represents what the \texttt{MqttBroker} will do upon receiving the \texttt{connect} message, i.e. add the \texttt{MqttClient} to it's set of peers and send back to the sender an acknowledgement message. With the third rule, the \texttt{MqttClient} processes any incoming acknowledgement message by setting its \texttt{peer} attribute with the senders identifier.

\begin{figure}[t]
\begin{Verbatim}
rl [mqtt/C/send-connect] :
    < Me : MqttClient | peer : nothing, cmdList : connect(B); CMDL, Atrs >
    =>
    < Me : MqttClient | peer : nothing, cmdList : CMDL, Atrs > (to B from Me : connect(B)) .

rl [mqtt/B/accept-connect] : 
    < Me : MqttBroker | peers : Ps, Atrs > (to Me from O : connect(Me)) 
    =>
    < Me : MqttBroker | peers : insert(O, Ps), Atrs > (to O from Me : connack) .

rl [mqtt/C/recv-connack] : 
    < Me : MqttClient | peer : nothing, Atrs > (to Me from O : connack)
    =>
    < Me : MqttClient | peer : O, Atrs > .
\end{Verbatim}
\caption{Subset of actor rules from the MQTT Maude specification, formalizing the semantics of a client connecting to a broker.}
\label{fig:mqtt-actor-rules}
\end{figure}

\begin{comment}
\victor{[REM4ESORICS]
The initial configuration, represented in Figure \ref{fig:mqtt-intial-conf}, has three objects: two clients (with identifiers \texttt{c1} and \texttt{c2} respectively) and one broker (with identifier \texttt{b}). Given the commands in the \texttt{cmdList} attribute of each client, what will happen is: 1) both clients will connect to the broker, 2) client \texttt{c1} will subscribe to topic \texttt{temperature} and, 3) client \texttt{c2} will publish value \texttt{34} on that same topic. In the end, client \texttt{c1} will receive a value published by client \texttt{c2} regarding the temperature, storing the last received value (34) in attribute \texttt{lastRecv}.
For the dialect examples in this work, we use this initial configuration (state). %The complete specification file is available in the repository \footnote{https://github.com/v1ct0r-byte/dialects}. 
}

\begin{figure}[t]
\begin{Verbatim}
< c1 : MqttClient | peer : nothing, 
                    cmdList : (connect(b) ; 
                               subscribe("temp")), 
                    lastRecv : empty > 
< c2 : MqttClient | peer : nothing, 
                    cmdList : 
                        (connect(b) ; 
                         publish("temp", "34")),
                    lastRecv : empty > 
< b : MqttBroker | peers : empty, 
                   subscribers : empty >
\end{Verbatim}
\caption{Initial MQTT configuration for experiments.}
\label{fig:mqtt-intial-conf}
\end{figure}
\end{comment}
\end{example}

